FlashFFTConv: Efficient Convolutions for Long Sequences with Tensor Cores

Convolution models with long filters have demonstrated state-of-the-art reasoning abilities in many long-sequence tasks but lag behind the most optimized Transformers in wall-clock time. A major bottleneck is the Fast Fourier Transform (FFT)--which allows long convolutions to run in $O(N logN)$ time in sequence length $N$ but has poor hardware utilization. In this paper, we study how to optimize the FFT convolution. We find two key bottlenecks: the FFT does not effectively use specialized matrix multiply units, and it incurs expensive I/O between layers of the memory hierarchy. In response, we propose FlashFFTConv. FlashFFTConv uses a matrix decomposition that computes the FFT using matrix multiply units and enables kernel fusion for long sequences, reducing I/O. We also present two sparse convolution algorithms--1) partial convolutions and 2) frequency-sparse convolutions--which can be implemented simply by skipping blocks in the matrix decomposition, enabling further opportunities for memory and compute savings. FlashFFTConv speeds up exact FFT convolutions by up to 7.93$\times$ over PyTorch and achieves up to 4.4$\times$ speedup end-to-end. Given the same compute budget, FlashFFTConv allows Hyena-GPT-s to achieve 2.3 points better perplexity on the PILE and M2-BERT-base to achieve 3.3 points higher GLUE score--matching models with twice the parameter count. FlashFFTConv also achieves 96.1% accuracy on Path-512, a high-resolution vision task where no model had previously achieved better than 50%. Furthermore, partial convolutions enable longer-sequence models--yielding the first DNA model that can process the longest human genes (2.3M base pairs)--and frequency-sparse convolutions speed up pretrained models while maintaining or improving model quality.

==> tables/convolution_benchmark_benchmark.tex <==
\begin{table}[t]
    \centering
    \small
    \caption{Top: Time ($\downarrow$) to compute the backward pass of a convolution with \sysname in milliseconds on A100. Bottom: Ablations removing specific optimizations. Batch size 64, hidden dimension 768. $p$ indicates the order of the Monarch decomposition.}
    \label{tab:convolution_benchmark_backward}
    \begin{tabular}{rccccccccc}
    \toprule
                                     & \multicolumn{2}{c}{\textbf{$p=2$}} & \multicolumn{4}{c}{\textbf{$p=3$}}        & \multicolumn{3}{c}{\textbf{$p=4$}} \\
                                     \cmidrule(){2-3} \cmidrule(lr){4-7} \cmidrule(lr){8-10}
          Sequence Length   & \textbf{256}            & \textbf{1K}            & \textbf{4K}  & \textbf{8K}  & \textbf{16K}   & \textbf{32K}  & \textbf{1M}           & \textbf{2M}           & \textbf{4M}    \\ \midrule
    PyTorch                 & 1.19                    & 2.92                   & 17.4         & 34.8         & 71.2           & 161.3         & 5,999.4               & 12,065.3              & 25,113.6       \\
    \sysname                & \textbf{0.18}           & \textbf{0.67}          & \textbf{4.1} & \textbf{8.9} & \textbf{32.0}  & \textbf{86.8} & \textbf{3,429.8}      & \textbf{7,181.7}      & \textbf{14,499.8}      \\ \bottomrule
    \end{tabular}
\end{table}
